Minimal Work: A Grasp Quality Metric for Deformable Hollow Objects

Robot grasping of deformable hollow objects such as plastic bottles and cups is challenging as the grasp should resist disturbances while minimally deforming the object so as not to damage it or dislodge liquids. We propose minimal work as a novel grasp quality metric that combines wrench resistance and the object deformation. We introduce an efficient algorithm to compute required work to resist an external wrench for a manipulation task by solving a linear program. The algorithm first computes the minimum required grasp force and an estimation of the gripper jaw displacements based on the object deformability at different locations measured with physical experiments. The work done by the jaws is the product of the grasp force and the displacements. The grasp quality metric is computed based on the required work under perturbations of grasp poses to address uncertainties in actuation. We collect 460 physical grasps with a UR5 robot and a Robotiq gripper. Physical experiments suggest the minimal work quality metric reaches 74.2% balanced accuracy and is up to 24.2% higher than classical wrench-based quality metrics, where the balanced accuracy is the raw accuracy normalized by the number of successful and failed real-world grasps.

==> sections/0-preamble.tex <==
% TODO: Remove unneeded packages
\ProvidesPackage{mysty}[2011/02/23 v1.0 My own macros]

\usepackage{subfiles}
\usepackage{cite}
\usepackage[pdftex]{graphicx}
% \usepackage{graphicx}
% \usepackage[export]{adjustbox}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage[section]{placeins}
\usepackage{tabularx}
\usepackage{array}
%\usepackage[top=0.5cm, bottom=0.5cm, left=0.5cm, right=0.5cm, columnsep=0.75cm]{geometry}
\setlength{\extrarowheight}{.3em} % add space for table

% \usepackage{flushend} % a package for last page

%\usepackage{mathtools}
%\usepackage{tabls}
\usepackage{algorithmic}
\usepackage{array}
\usepackage{subfig}
\usepackage{float}
%\usepackage{dblfloatfix} %\begin{figure*}[!b]% double column figures in the bottom
\usepackage{url}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage{amsfonts}
\usepackage[boxed,linesnumbered]{algorithm2e}
\usepackage{xfrac}
\usepackage{fix-cm}  % To avoid warnings 'font shape not available' with sfrac
\usepackage{wrapfig}
\usepackage{color}  % Use: \color[rgb]{1,1,1}
\usepackage{tikz}
\usetikzlibrary{calc,arrows,positioning,matrix,fit,shapes,tikzmark,scopes} 
\usepackage{tikz-3dplot}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usepackage{makecell}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{siunitx}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%variables
%\newcommand\wone{23}
%\newcommand\wtwo{20}
\newcommand\wone{21}
\newcommand\wtwo{15}
\newcommand\wthree{17}


\newcommand\hpone{4.5}
\newcommand\hptwo{3.2}
\newcommand\hpthree{3.5}


\newcommand\taon{7}
\newcommand\tatw{8}
\newcommand\tatr{2.3}
\newcommand\tafo{7.3}


\newcommand\tbon{6.5}
\newcommand\tbtw{7.6}
\newcommand\tbtr{5}
\newcommand\tbfo{7.4}

\newcommand\hi{35mm}
\newcommand\his{25mm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%% FIG PATH %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\figbase{fig/def-adj-0.3}
\newcommand\figbasepa{\figbase/obj-def/pdf/}
\newcommand\figbasepb{\figbase/GWS-vol/pdf/}
\newcommand\figbasepc{\figbase/GWS-eps/pdf/}
\newcommand\figbasepd{\figbase/GWS-eps-min-work/pdf/}
\newcommand\figbasepe{\figbase/lift-up/min-force/pdf/}
\newcommand\figbasepf{\figbase/lift-up/min-work/pdf/}
\newcommand\figbasepg{\figbase/lift-up-rot-x/min-force/pdf/}
\newcommand\figbaseph{\figbase/lift-up-rot-x/min-work/pdf/}
\newcommand\figbasepi{\figbase/lift-up-rot-y/min-force/pdf/}
\newcommand\figbasepj{\figbase/lift-up-rot-y/min-work/pdf/}
\newcommand\figbasepk{\figbase/lift-up-rot-xyz/min-force/pdf/}
\newcommand\figbasepl{\figbase/lift-up-rot-xyz/min-work/pdf/}

\newcommand\figa{fig1}
\newcommand\figb{fig3}
\newcommand\figc{fig5}
\newcommand\figd{fig10}
\newcommand\fige{fig12}
\newcommand\figf{fig13}
\newcommand\figg{fig14}

\renewcommand{\t}{\boldsymbol{t}} % task
\newcommand{\f}{\boldsymbol{f}} % friction
\newcommand{\F}{\mathcal{F}} % friction set
\newcommand{\fperp}{\boldsymbol{f}_\perp} % wrench impressed by pressure
\newcommand{\x}{\boldsymbol{x}} % frictiosn
\newcommand{\work}{W} 

%\newcommand\figh{fig11}
%\newcommand\figi{fig23}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CUSTOM COMMANDS
%\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
%\newcolumntype{N}{@{}m{0pt}@{}}
%\renewcommand\theadfont{\bfseries\normalsize}
%\renewcommand\theadgape{}
%\setcellgapes{2pt}
% Commands for comments
% Adjust these for final version/removal of parts
\def\myfinal{yep}  % Uncomment this for final version. Hides comments.
\newif\ifremove   % Comment out one of following 2 lines:
\removetrue     % Shows parts marked with \ifremove
%\removefalse  % Hides parts marked with \ifremove

\def\mysum#1{\ifx\myfinal\undefined\textcolor{gray}{Summary: #1}\par\fi}
\def\mytop{\mysum}
\def\mydo#1{\ifx\myfinal\undefined\textcolor{blue}{#1}\par\fi}
\def\mydel#1{\ifx\myfinal\undefined\textcolor{red}{#1}\par\fi}

% Shotcut commands
\def\sref#1{Sec.~\ref{#1}}
\def\fref#1{Fig.~\ref{#1}}
\def\eref#1{Eqn.~\eqref{#1}}
\def\tref#1{Table~\ref{#1}}
\def\mysub#1{\textit{\protect\subref{#1}}}
\def\mymod#1{\textcolor{black}{#1}}

\def\eg{e.g.\ }
\def\ie{i.e.\ }

\def\mysubspace{\hspace{0.2em}} % Defaults Space btwen subfloats
\def\myitemsep{\itemsep0pt}
% w/h of (tikz) figures
\newlength\w
\newlength\h

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\eq}{Equation}
\newcommand{\fig}{Fig.}

%%%%
% funtions
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcount\colveccount
\newcommand*\colvec[1]{
	\global\colveccount#1
	\begin{pmatrix}
		\colvecnext
	}
	\def\colvecnext#1{
		#1
		\global\advance\colveccount-1
		\ifnum\colveccount>0
		\\
		\expandafter\colvecnext
		\else
	\end{pmatrix}
	\fi
}
% parameters
\newcommand{\boldsigma}{\boldsymbol{\sigma}}
\newcommand{\boldn}{\boldsymbol{n}}
\newcommand{\boldm}{\boldsymbol{m}}
\newcommand{\surface}{\mathcal{S}}
\newcommand{\tangent}{T_{p}\mathcal{S}}
\newcommand{\pressure}{\mathcal{P}}
%\newcommand{\lcor}{l_\text{COR}}
\newcommand{\vp}{\boldsymbol{v}_p}
\newcommand{\vo}{\boldsymbol{v}_o}
\newcommand{\boldomega}{\boldsymbol{\omega}}
\newcommand{\projvp}{\tilde{\boldsymbol{v}}_p}
\newcommand{\boldf}{\boldsymbol{f}}
\newcommand{\boldtau}{\boldsymbol{\tau}}
\newcommand{\boldw}{\boldsymbol{w}}
%\newcommand{\boldt}{\boldsymbol{T}}
\newcommand{\wrench}{{\mathsf{w}}}
\newcommand{\twist}{{\mathsf{t}}}
% \newcommand{\boldw}{\boldsymbol{\mathsf{w}}}
% \newcommand{\boldW}{\boldsymbol{\mathsf{W}}}
\newcommand{\boldt}{\boldsymbol{\mathsf{t}}}
\newcommand{\errorwrenchi}{{\varepsilon}_{\mathsf{w}_i}}
\newcommand{\errortwisti}{{\varepsilon}_{\mathsf{t}_i}}
\newcommand{\errorwrench}{\boldsymbol{\varepsilon}_{\mathsf{w}}}
\newcommand{\errortwist}{\boldsymbol{\varepsilon}_{\mathsf{t}}}
\newcommand{\origin}{\mathcal{O}}
\newcommand{\mbeq}{\overset{!}{=}}
\newcommand{\matr}[1]{\mathbf{#1}} 
\newcommand*\mean[1]{\bar{#1}} \newcommand{\parallelsum}{\mathbin{\!/\mkern-5mu/\!}}
\renewcommand{\v}{\boldsymbol{v}}
\newcommand{\m}{\boldsymbol{m}}

% \newcommand{\w}{\boldsymbol{w}}

%\newcommand{\lIAR}{l_{\text{IAR}}}
\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% SYMBOLS

\def\u#1{\,\textup{#1}}
\def\V#1{\ensuremath{\mathbf{#1}}}
\def\mym#1{\ensuremath{#1}}
\def\sDef{\mym{\delta}}
\def\sFeat{\mym{\mathcal{F}}}
\def\sForce{\mym{F}}
\def\sN{\mym{\V{n}}}
\def\sNbh{\mym{\mathcal{N}}}
\def\sProb{\mym{p}}
\def\sScore{\mym{\mathcal{S}}}
\def\sX{\@ifnextchar[{\@sXFrame}{\mym{\V{X}}}}

\def\ftNrm{\hat{\sFeat}^{i}} %\ftNrm
\def\ftScLow{\tilde{\sFeat}^{i}} %\ftScLow
\def\ftScbLow{\tilde{\sFeat}^{i,(1)}} %\ftScbLow


==> sections/figures/grasp_score_rot1.tex <==
\begin{figure*}
	\centering	
%%%%%%%%%%%%%%%%%%%%%%%%% rot 1 %%%%%%%%%%%%%%%%%%%%%%%%%%
    % robust
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/w5/r1r.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/mustard/r1r.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/shampoo/r1r.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/box/r1r.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/cup/r1r.png} }}% 
	
    %  min force 
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/w5/r1mf.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/mustard/r1mf.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/shampoo/r1mf.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/box/r1mf.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/cup/r1mf.png} }}% 
	
    %  min work 
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/w5/r1mw.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/mustard/r1mw.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/shampoo/r1mw.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/box/r1mw.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/cup/r1mw.png} }}% 
	
	\caption{rot1}
	\label{fig:metrics_rot1}
\end{figure*}


==> sections/figures/grasp_score_rot2.tex <==
\begin{figure}
	\centering	
%%%%%%%%%%%%%%%%%%%%%%%%% rot 2 %%%%%%%%%%%%%%%%%%%%%%%%%%
    % robust
% 	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/w5/r2r.png} }}% 	
% 	\qquad
% 	\hspace{-\hpone em}
% 	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/mustard/r2r.png} }}% 	
% 	\qquad
% 	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[height=35 mm,trim={4cm  5cm 0cm 1cm},clip]{fig/shampoo/r2r.png} }}% 	
	\qquad
% 	\hspace{-\hpone em}
% 	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/box/r2r.png} }}% 	
% 	\qquad
% 	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[height=35 mm,trim={4cm  5cm 0cm 1cm},clip]{fig/cup/r2r.png} }}% 
	
%     %  min force 
% 	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/w5/r2mf.png} }}% 	
% 	\qquad
% 	\hspace{-\hpone em}
% 	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/mustard/r2mf.png} }}% 	
% 	\qquad
% 	\hspace{-\hpone em}
% 	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/shampoo/r2mf.png} }}% 	
% 	\qquad
% 	\hspace{-\hpone em}
% 	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/box/r2mf.png} }}% 	
% 	\qquad
% 	\hspace{-\hpone em}
% 	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/cup/r2mf.png} }}% 
	
    %  min work 
% 	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/w5/r2mw.png} }}% 	
% 	\qquad
% 	\hspace{-\hpone em}
% 	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/mustard/r2mw.png} }}% 	
% 	\qquad
% 	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[height=35 mm,trim={4cm  5cm 0cm 1cm},clip]{fig/shampoo/r2mw.png} }}% 	
	\qquad
% 	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 0cm}]{fig/box/r2mw.png} }}% 	
% 	\qquad
% 	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[height=35 mm,trim={4cm  5cm 0cm 1cm},clip]{fig/cup/r2mw.png} }}% 
	
	\caption{Example minimal force and minimal work grasps for a rotation around the $y$-axis. Content might spill with proposed grasps since the object deformation is not strictly prevented. }
	\label{fig:metrics_rot2}
\end{figure}


==> sections/figures/grasp_score_row.tex <==
\begin{figure*}
	\centering	
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[height=\hi,trim={8cm 0 2cm 0},clip]{fig/w5/stiffness.png} }}% 
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[height=\hi,trim={8cm 0 1cm 0},clip]{fig/w5/tr}}}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[height=\hi,trim={5cm 0 1cm 0},clip]{fig/w5/tmf.png} }}% 	
	\hspace{-\hpone em}
	\qquad
	\subfloat[]{{\includegraphics[height=\hi,trim={5cm 0 1cm 0},clip]{fig/w5/tmw.png} }}% 	
	\qquad
	\hspace{-4.5 em}
	\subfloat[]{{\includegraphics[height=\hi,trim={3cm 0 0cm 0},clip]{fig/w5/r1r.png} }}% 	
	\qquad
	\hspace{-3 em}
	\subfloat[]{{\includegraphics[height=\hi,trim={4cm 0 0cm 0},clip]{fig/w5/r1mf.png} }}% 	
	\hspace{-3 em}
	\qquad
	\subfloat[]{{\includegraphics[height=\hi,trim={4cm 0 0cm 0},clip]{fig/w5/r1mw.png} }}% 	
% 	\qquad
% 	\hspace{-2.2 em}
% 	\subfloat[]{{\includegraphics[height=25 mm,trim={3cm 0 0cm 0},clip]{fig/w5/r2mf.png} }}% 	
% 	\qquad
% 	\hspace{-2.2 em}	
% 	\subfloat[]{{\includegraphics[height=25 mm,trim={3cm 0 0cm 0},clip]{fig/w5/r2mf.png} }}% 	
% 	\hspace{-2.2 em}
% 	\qquad
% 	\subfloat[]{{\includegraphics[height=25 mm,trim={3cm 0 0cm 0},clip]{fig/w5/r2mw.png} }}% 
	
%%%%%%%%%%%%%%%%%%%%% mustard
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[height=\hi,trim={8cm 0 2cm 0},clip]{fig/mustard/stiffness.png} }}% 
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[height=\hi,trim={8cm 0 1cm 0},clip]{fig/mustard/tr}}}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[height=\hi,trim={5cm 0 1cm 0},clip]{fig/mustard/tmf.png} }}% 	
	\hspace{-\hpone em}
	\qquad
	\subfloat[]{{\includegraphics[height=\hi,trim={5cm 0 1cm 0},clip]{fig/mustard/tmw.png} }}% 	
	\qquad
	\hspace{-4.5 em}
	\subfloat[]{{\includegraphics[height=\hi,trim={3cm 0 0cm 0},clip]{fig/mustard/r1r.png} }}% 	
	\qquad
	\hspace{-3 em}
	\subfloat[]{{\includegraphics[height=\hi,trim={4cm 0 0cm 0},clip]{fig/mustard/r1mf.png} }}% 	
	\hspace{-3 em}
	\qquad
	\subfloat[]{{\includegraphics[height=\hi,trim={4cm 0 0cm 0},clip]{fig/mustard/r1mw.png} }}% 	
% 	\qquad
% 	\hspace{-2.2 em}
% 	\subfloat[]{{\includegraphics[height=\hi,trim={3cm 0 0cm 0},clip]{fig/mustard/r2mf.png} }}% 	
% 	\qquad
% 	\hspace{-2.2 em}	
% 	\subfloat[]{{\includegraphics[height=\hi,trim={3cm 0 0cm 0},clip]{fig/mustard/r2mf.png} }}% 	
% 	\hspace{-2.2 em}
% 	\qquad
% 	\subfloat[]{{\includegraphics[height=\hi,trim={3cm 0 0cm 0},clip]{fig/mustard/r2mw.png} }}% 
	
%%%%%%%%%%%%%%%%%%%%% shampoo
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[height=\hi,trim={8cm 0 2cm 0},clip]{fig/shampoo/stiffness.png} }}% 
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[height=\hi,trim={8cm 0 1cm 0},clip]{fig/shampoo/tr}}}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[height=\hi,trim={5cm 0 1cm 0},clip]{fig/shampoo/tmf.png} }}% 	
	\hspace{-\hpone em}
	\qquad
	\subfloat[]{{\includegraphics[height=\hi,trim={5cm 0 1cm 0},clip]{fig/shampoo/tmw.png} }}% 	
	\qquad
	\hspace{-4.5 em}
	\subfloat[]{{\includegraphics[height=\hi,trim={3cm 0 0cm 0},clip]{fig/shampoo/r1r.png} }}% 	
	\qquad
	\hspace{-3 em}
	\subfloat[]{{\includegraphics[height=\hi,trim={4cm 0 0cm 0},clip]{fig/shampoo/r1mf.png} }}% 	
	\hspace{-3 em}
	\qquad
	\subfloat[]{{\includegraphics[height=\hi,trim={4cm 0 0cm 0},clip]{fig/shampoo/r1mw.png} }}% 	
% 	\qquad
% 	\hspace{-2.2 em}
% 	\subfloat[]{{\includegraphics[height=\hi,trim={3cm 0 0cm 0},clip]{fig/shampoo/r2mf.png} }}% 	
% 	\qquad
% 	\hspace{-2.2 em}	
% 	\subfloat[]{{\includegraphics[height=\hi,trim={3cm 0 0cm 0},clip]{fig/shampoo/r2mf.png} }}% 	
% 	\hspace{-2.2 em}
% 	\qquad
% 	\subfloat[]{{\includegraphics[height=\hi,trim={3cm 0 0cm 0},clip]{fig/shampoo/r2mw.png} }}% 	
	
%%%%%%%%%%%%%%%%%%%%% box
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[height=\hi,trim={8cm 0 2cm 0},clip]{fig/box/stiffness.png} }}% 
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[height=\hi,trim={8cm 0 1cm 0},clip]{fig/box/tr}}}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[height=\hi,trim={5cm 0 1cm 0},clip]{fig/box/tmf.png} }}% 	
	\hspace{-\hpone em}
	\qquad
	\subfloat[]{{\includegraphics[height=\hi,trim={5cm 0 1cm 0},clip]{fig/box/tmw.png} }}% 	
	\qquad
	\hspace{-4.5 em}
	\subfloat[]{{\includegraphics[height=\hi,trim={3cm 0 0cm 0},clip]{fig/box/r1r.png} }}% 	
	\qquad
	\hspace{-3 em}
	\subfloat[]{{\includegraphics[height=\hi,trim={4cm 0 0cm 0},clip]{fig/box/r1mf.png} }}% 	
	\hspace{-3 em}
	\qquad
	\subfloat[]{{\includegraphics[height=\hi,trim={4cm 0 0cm 0},clip]{fig/box/r1mw.png} }}% 	
% 	\qquad
% 	\hspace{-2.2 em}
% 	\subfloat[]{{\includegraphics[height=\hi,trim={3cm 0 0cm 0},clip]{fig/box/r2mf.png} }}% 	
% 	\qquad
% 	\hspace{-2.2 em}	
% 	\subfloat[]{{\includegraphics[height=\hi,trim={3cm 0 0cm 0},clip]{fig/box/r2mf.png} }}% 	
% 	\hspace{-2.2 em}
% 	\qquad
% 	\subfloat[]{{\includegraphics[height=\hi,trim={3cm 0 0cm 0},clip]{fig/box/r2mw.png} }}% 	
	
	
%%%%%%%%%%%%%%%%%%%%% cup
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[height=\hi,trim={8cm 0 2cm 0},clip]{fig/cup/stiffness.png} }}% 
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[height=\hi,trim={8cm 0 1cm 0},clip]{fig/cup/tr}}}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[height=\hi,trim={5cm 0 1cm 0},clip]{fig/cup/tmf.png} }}% 	
	\hspace{-\hpone em}
	\qquad
	\subfloat[]{{\includegraphics[height=\hi,trim={5cm 0 1cm 0},clip]{fig/cup/tmw.png} }}% 	
	\qquad
	\hspace{-4.5 em}
	\subfloat[]{{\includegraphics[height=\hi,trim={3cm 0 0cm 0},clip]{fig/cup/r1r.png} }}% 	
	\qquad
	\hspace{-3 em}
	\subfloat[]{{\includegraphics[height=\hi,trim={4cm 0 0cm 0},clip]{fig/cup/r1mf.png} }}% 	
	\hspace{-3 em}
	\qquad
	\subfloat[]{{\includegraphics[height=\hi,trim={4cm 0 0cm 0},clip]{fig/cup/r1mw.png} }}% 	
% 	\qquad
% 	\hspace{-2.2 em}
% 	\subfloat[]{{\includegraphics[height=\hi,trim={3cm 0 0cm 0},clip]{fig/cup/r2mf.png} }}% 	
% 	\qquad
% 	\hspace{-2.2 em}	
% 	\subfloat[]{{\includegraphics[height=\hi,trim={3cm 0 0cm 0},clip]{fig/cup/r2mf.png} }}% 	
% 	\hspace{-2.2 em}
% 	\qquad
% 	\subfloat[]{{\includegraphics[height=\hi,trim={3cm 0 0cm 0},clip]{fig/cup/r2mw.png} }}% 	
	
% 	\subfloat[Stiffness map.]{{\includegraphics[width=50 mm]{fig/mustard/stiffness.png} }}% 	
% 	\qquad
% 	\hspace{-\hpone em}
% 	\subfloat[Wrench resistance metric.]{{\includegraphics[width=50 mm]{fig/mustard/robust.png} }}% 	
% 	\qquad
% 	\hspace{-\hpone em}
% 	\subfloat[Minimal force metric.]{{\includegraphics[width=50 mm]{fig/mustard/min_force.png} }}% 	
% 	\hspace{-\hpone em}
% 	\qquad
% 	\subfloat[Minimal work metric.]{{\includegraphics[width=50 mm]{fig/mustard/min_work.png} }}% 	
% 	\hspace{-\hpone em}
	
% 	\subfloat[Stiffness map.]{{\includegraphics[width=50 mm]{fig/shampoo/stiffness.png} }}% 	
% 	\qquad
% 	\hspace{-\hpone em}
% 	\subfloat[Wrench resistance metric.]{{\includegraphics[width=50 mm]{fig/shampoo/robust.png} }}% 	
% 	\qquad
% 	\hspace{-\hpone em}
% 	\subfloat[Minimal force metric.]{{\includegraphics[width=50 mm]{fig/shampoo/min_force.png} }}% 	
% 	\hspace{-\hpone em}
% 	\qquad
% 	\subfloat[Minimal work metric.]{{\includegraphics[width=50 mm]{fig/shampoo/min_work.png} }}% 	
% 	\hspace{-\hpone em}

	\caption{Quality of grasps with three metrics for a lift up task. The proposed minimal work metric is able to select good grasps without dislodge fluids while resisting disturbances. WILL ADD: images of real objects and scalar of the stiffness map.}
	\label{fig:metrics}
\end{figure*}


==> sections/figures/grasp_scores.tex <==
\begin{figure*}
	\centering	
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/w5/stiffness.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/mustard/stiffness.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/shampoo/stiffness.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/box/stiffness.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/cup/stiffness.png} }}% 	

%%%%%%%%%%%%%%%%%%%%%%%%% lift up %%%%%%%%%%%%%%%%%%%%%%%%%%
    % lift up robust
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/w5/tr.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/mustard/tr.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/shampoo/tr.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/box/tr.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/cup/tr.png} }}% 
	
    % lift up min force 
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/w5/tmf.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/mustard/tmf.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/shampoo/tmf.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/box/tmf.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/cup/tmf.png} }}% 
	
    % lift up min work 
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/w5/tmw.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/mustard/tmw.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/shampoo/tmw.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/box/tmw.png} }}% 	
	\qquad
	\hspace{-\hpone em}
	\subfloat[]{{\includegraphics[width=40 mm,trim={0cm  0cm 0cm 1cm}]{fig/cup/tmw.png} }}% 
	

	
	\caption{Quality of grasps with three metrics for a lift up task. The proposed minimal work metric is able to select good grasps without dislodge fluids while resisting disturbances. WILL ADD: images of real objects and scalar of the stiffness map.}
	\label{fig:metrics}
\end{figure*}

